PrimA6D: Rotational Primitive Reconstruction for Enhanced and Robust 6D Pose Estimation

In this paper, we introduce a rotational primitive prediction based 6D object pose estimation using a single image as an input. We solve for the 6D object pose of a known object relative to the camera using a single image with occlusion. Many recent state-of-the-art (SOTA) two-step approaches have exploited image keypoints extraction followed by PnP regression for pose estimation. Instead of relying on bounding box or keypoints on the object, we propose to learn orientation-induced primitive so as to achieve the pose estimation accuracy regardless of the object size. We leverage a Variational AutoEncoder (VAE) to learn this underlying primitive and its associated keypoints. The keypoints inferred from the reconstructed primitive image are then used to regress the rotation using PnP. Lastly, we compute the translation in a separate localization module to complete the entire 6D pose estimation. When evaluated over public datasets, the proposed method yields a notable improvement over the LINEMOD, the Occlusion LINEMOD, and the YCB-Video dataset. We further provide a synthetic-only trained case presenting comparable performance to the existing methods which require real images in the training phase.

==> tab_ablation.tex <==
\begin{table}[!b]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|cc|c|ccc}
    \hline
     methods & PVNet\cite{pvnet-2019-cvpr} & PrimA6D-S & PrimA6D-SR & w/o GAN & 10\% & 20\% & 30\% \\ \hline \hline
     ape         & & & & & & & \\ \hline
     can         & & & & & & & \\ \hline
     cat         & & & & & & & \\ \hline
     duck        & & & & & & & \\ \hline
     driller     & & & & & & & \\ \hline
     eggbox*     & & & & & & & \\ \hline
     glue*       & & & & & & & \\ \hline
     holepuncher & & & & & & & \\ \hline \hline
     average     & & & & & & & \\ \hline
  \end{tabular}
  }
  \vspace{0.1mm}
  \caption{Ablation study on Occlusion LINEMOD dataset.}
  \label{tab:ablation}
\end{table}


==> tab_occlusion.tex <==
\begin{figure*}[!t]
  \begin{minipage}{0.7\textwidth}
  \scriptsize{
  \subfigure[ADD(-S) over Occlusion LINEMOD]{
    \label{tab:occ.add}
    \begin{tabular}{c|ccccc|ccc}
      \hline
                methods & Tekin & PoseCNN & Oberweger\cite{oberweger2018making} & Pix2Pose & PVNet & w/o GAN & PrimA6D-S & PrimA6D-SR \\ \hline \hline
           ape$^\dagger$& 2.48  & 9.6   & 17.6  & 22    & 15.81 & 2.75 & 28.71 & \B{37.35} \\ \hline
           can          & 17.48 & 45.2  & 53.9  & 44.7  & 63.3  & 5.47 & 61.88 & \B{67.19} \\ \hline
           cat$^\dagger$& 0.67  & 0.93  & 3.31  & 22.7  & 16.68 & 1.68 & 40.43 & \B{44.65} \\ \hline
          duck$^\dagger$& 1.14  & 19.6  & 19.2  & 15    & 25.24 & 10.87 &39.28 & \B{50.65} \\ \hline
           driller      & 7.66  & 41.4  & 62.4  & 44.7  & 65.65 & 9.71 & 70.42 & \B{74.87} \\ \hline
           eggbox*      & -     & 22    & 25.9  & 25.2  & 50.17 & 7.02 & 54.31 & \B{66.01} \\ \hline
           glue*        & 10.08 & 38.5  & 39.6  & 32.4  & 49.62 & 7.72 & 71.03 & \B{73.02} \\ \hline
   holepuncher$^\dagger$& 5.45  & 22.1  & 21.3  & 49.5  & 39.67 & 12.41 & 46.19 & \B{64.38} \\ \hline \hline
           average      & 6.42  & 24.92 & 30.40 & 32.00 & 40.77 & 7.20 & 51.53 & \B{59.77} \\ \hline
    \end{tabular}
  }%subfigure
  }%scriptsize
  \end{minipage}\hfill
  %\begin{minipage}{0.2\textwidth}
  %  	\centering
  %  	\subfigure[Ape]{
  %  		\includegraphics[width=\columnwidth]{figs/ape} % abl.bb.APE
  %      \label{fig:abl.bb.ape}
  %  	}%
  %\end{minipage}\\
  \begin{minipage}{0.54\textwidth}
  \resizebox{\linewidth}{!}{
    \subfigure[2D Projection error over Occlusion LINEMOD]{
    \label{tab:occ.2dp}
  \begin{tabular}{c|cccc|cc}
    \hline
             methods & Tekin & PoseCNN & Oberweger & PVNet &  PrimA6D-S & PrimA6D-SR \\ \hline \hline
        ape$^\dagger$& 7.01 & 34.6  & \B{69.9}  & 69.14 &  56.58 & 62.64 \\ \hline
        can          & 11.2 & 15.1  & 82.6  & \B{86.09} &  69.26 & 76.8 \\ \hline
        cat$^\dagger$& 3.62 & 10.4  & 65.1  & \B{65.12} &  54.33 & 58.8 \\ \hline
       duck$^\dagger$& 5.07 & 31.8  & 61.4  & 61.44     &  64.74 & \B{67.36} \\ \hline
        driller      & 1.4  & 7.4   & \B{73.8}  & 73.06 &  59.55 & 61.28 \\ \hline
        eggbox*      & -    & 1.9   & 13.1  & 8.43      &  8.53  & \B{16.48} \\ \hline
        glue*        & 4.7  & 13.8  & 54.9  & 55.37 &  51.83 & \B{57.38}  \\ \hline
holepuncher$^\dagger$& 8.26 & 23.1  & 66.4  & \B{69.84}     &  50.82 & 67.76 \\ \hline \hline
        average      & 5.89 & 17.26 & 60.90 & \B{61.06} &  51.96 & 58.56 \\ \hline
  \end{tabular}
  }
  }
  \end{minipage}\hfill
  %\begin{minipage}{0.43\textwidth}
  %  \subfigure[Benchvise]{
  %    \includegraphics[width=0.48\columnwidth]{figs/benchvise}
  %    \label{fig:abl.bb.benchvise}
  %  }
  %  \subfigure[Eggbox]{
  %    \includegraphics[width=0.48\columnwidth]{figs/eggbox}
  %    \label{fig:abl.bb.eggbox}
  %  }
  %\end{minipage}
  \vspace{0.1mm}
  \caption{The accuracy in terms of the \subref{tab:occ.add} ADD(-S) metric and \subref{tab:occ.2dp} 2D projection error for our method and baseline methods on the Occlusion LINEMOD dataset. All values are imported from \cite{pvnet-2019-cvpr} except pix2pose. Symmetrical objects are marked with an asterisk (*) and small objects are marked with $^\dagger$. \subref{fig:abl.bb.ape}, \subref{fig:abl.bb.benchvise} and \subref{fig:abl.bb.eggbox} illustrate the 6D pose estimation performance change according to the accuracy of bounding-box.}
  \label{fig:occ_ablbb}
\end{figure*}

